Geometric Matrix Completion with Recurrent Multi-Graph Neural Networks

Matrix completion models are among the most common formulations of recommender systems. Recent works have showed a boost of performance of these techniques when introducing the pairwise relationships between users/items in the form of graphs, and imposing smoothness priors on these graphs. However, such techniques do not fully exploit the local stationarity structures of user/item graphs, and the number of parameters to learn is linear w.r.t. the number of users and items. We propose a novel approach to overcome these limitations by using geometric deep learning on graphs. Our matrix completion architecture combines graph convolutional neural networks and recurrent neural networks to learn meaningful statistical graph-structured patterns and the non-linear diffusion process that generates the known ratings. This neural network system requires a constant number of parameters independent of the matrix size. We apply our method on both synthetic and real datasets, showing that it outperforms state-of-the-art techniques.

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_0/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=-1.17515140687376,
point meta max=1.80726075219065,
colorbar style={ytick={-0.8,-0.4,2.22044604925031e-16,0.4,0.8,1.2,1.6},yticklabels={−0.8,−0.4,0.0,0.4,0.8,1.2,1.6}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_0_absolute_value/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
%colorbar,
%xtick = {0, 10, 19.5},
%xticklabels = {0,1,2},
%ytick = {0, 10, 19.5},
%yticklabels = {2,1,0},
%xticklabel pos=right,
%xlabel near ticks,
xtick=\empty,
ytick=\empty,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=0.00113467233532974,
point meta max=1.80726075219065,
colorbar style={ytick={0.2,0.4,0.6,0.8,1,1.2,1.4,1.6,1.8},yticklabels={0.2,0.4,0.6,0.8,1.0,1.2,1.4,1.6,1.8}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_0_absolute_value/filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_1/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
%colorbar,
xtick=\empty,
ytick=\empty,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=-1.47148430243088,
point meta max=1.62648426677333,
colorbar style={ytick={-1.2,-0.8,-0.4,-2.22044604925031e-16,0.4,0.8,1.2,1.6},yticklabels={−1.2,−0.8,−0.4,0.0,0.4,0.8,1.2,1.6}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_1_absolute_value/filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_10/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=-4.50155762210488,
point meta max=1.0730414724648,
colorbar style={ytick={-4.2,-3.6,-3,-2.4,-1.8,-1.2,-0.6,0,0.600000000000001},yticklabels={−4.2,−3.6,−3.0,−2.4,−1.8,−1.2,−0.6,0.0,0.6}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_10_absolute_value/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=0.000242071800994933,
point meta max=4.50155762210488,
colorbar style={ytick={0.5,1,1.5,2,2.5,3,3.5,4,4.5},yticklabels={0.5,1.0,1.5,2.0,2.5,3.0,3.5,4.0,4.5}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_11/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=-1.82848609327078,
point meta max=1.24083026846647,
colorbar style={ytick={-1.6,-1.2,-0.8,-0.4,0,0.400000000000001,0.800000000000001,1.2},yticklabels={−1.6,−1.2,−0.8,−0.4,0.0,0.4,0.8,1.2}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_11_absolute_value/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=0.00103769716996232,
point meta max=1.82848609327078,
colorbar style={ytick={0.2,0.4,0.6,0.8,1,1.2,1.4,1.6,1.8},yticklabels={0.2,0.4,0.6,0.8,1.0,1.2,1.4,1.6,1.8}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_12/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=-1.36086609452653,
point meta max=1.47707886122582,
colorbar style={ytick={-1.2,-0.9,-0.6,-0.3,0,0.3,0.6,0.9,1.2},yticklabels={−1.2,−0.9,−0.6,−0.3,0.0,0.3,0.6,0.9,1.2}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_12_absolute_value/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=0.00279612615258448,
point meta max=1.47707886122582,
colorbar style={ytick={0.15,0.3,0.45,0.6,0.75,0.9,1.05,1.2,1.35},yticklabels={0.15,0.30,0.45,0.60,0.75,0.90,1.05,1.20,1.35}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_13/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=-1.22716501707608,
point meta max=1.5989498064965,
colorbar style={ytick={-1.2,-0.8,-0.4,0,0.4,0.8,1.2},yticklabels={−1.2,−0.8,−0.4,0.0,0.4,0.8,1.2}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_13_absolute_value/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=0.00554088386670154,
point meta max=1.5989498064965,
colorbar style={ytick={0.2,0.4,0.6,0.8,1,1.2,1.4},yticklabels={0.2,0.4,0.6,0.8,1.0,1.2,1.4}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_14/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=-1.1147196700895,
point meta max=1.39026073186249,
colorbar style={ytick={-0.9,-0.6,-0.3,0,0.3,0.6,0.9,1.2},yticklabels={−0.9,−0.6,−0.3,0.0,0.3,0.6,0.9,1.2}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_14_absolute_value/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=0.00160678391796387,
point meta max=1.39026073186249,
colorbar style={ytick={0.15,0.3,0.45,0.6,0.75,0.9,1.05,1.2,1.35},yticklabels={0.15,0.30,0.45,0.60,0.75,0.90,1.05,1.20,1.35}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_15/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=-1.80715556977317,
point meta max=1.04023788907247,
colorbar style={ytick={-1.6,-1.2,-0.8,-0.4,2.22044604925031e-16,0.4,0.8},yticklabels={−1.6,−1.2,−0.8,−0.4,0.0,0.4,0.8}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_15_absolute_value/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=1.60664195621008e-06,
point meta max=1.80715556977317,
colorbar style={ytick={0.2,0.4,0.6,0.8,1,1.2,1.4,1.6,1.8},yticklabels={0.2,0.4,0.6,0.8,1.0,1.2,1.4,1.6,1.8}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_16/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=-1.75340907275677,
point meta max=1.35723394981409,
colorbar style={ytick={-1.6,-1.2,-0.8,-0.4,0,0.4,0.8,1.2},yticklabels={−1.6,−1.2,−0.8,−0.4,0.0,0.4,0.8,1.2}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_16_absolute_value/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=0.00297064462304044,
point meta max=1.75340907275677,
colorbar style={ytick={0.2,0.4,0.6,0.8,1,1.2,1.4,1.6},yticklabels={0.2,0.4,0.6,0.8,1.0,1.2,1.4,1.6}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_17/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=-1.29971612795524,
point meta max=2.14422303484753,
colorbar style={ytick={-1.2,-0.8,-0.4,0,0.4,0.8,1.2,1.6,2},yticklabels={−1.2,−0.8,−0.4,0.0,0.4,0.8,1.2,1.6,2.0}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_17_absolute_value/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=0.000501005830264205,
point meta max=2.14422303484753,
colorbar style={ytick={0.25,0.5,0.75,1,1.25,1.5,1.75,2},yticklabels={0.25,0.50,0.75,1.00,1.25,1.50,1.75,2.00}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_18/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=-0.736373286825116,
point meta max=1.5009402690921
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_18_absolute_value/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=0.00423087708055853,
point meta max=1.5009402690921,
colorbar style={ytick={0.2,0.4,0.6,0.8,1,1.2,1.4},yticklabels={0.2,0.4,0.6,0.8,1.0,1.2,1.4}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_19/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=-4.55369788967073,
point meta max=0.586730002518818,
colorbar style={ytick={-4.2,-3.6,-3,-2.4,-1.8,-1.2,-0.6,0},yticklabels={−4.2,−3.6,−3.0,−2.4,−1.8,−1.2,−0.6,0.0}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_19_absolute_value/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=8.52941887835112e-05,
point meta max=4.55369788967073,
colorbar style={ytick={0.5,1,1.5,2,2.5,3,3.5,4,4.5},yticklabels={0.5,1.0,1.5,2.0,2.5,3.0,3.5,4.0,4.5}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_1_absolute_value/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
%colorbar,
xtick=\empty,
ytick=\empty,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=0.00182024337306054,
point meta max=1.62648426677333,
colorbar style={ytick={0.2,0.4,0.6,0.8,1,1.2,1.4,1.6},yticklabels={0.2,0.4,0.6,0.8,1.0,1.2,1.4,1.6}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_1_absolute_value/filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_2/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=-0.980487978834722,
point meta max=1.81756495874524,
colorbar style={ytick={-0.8,-0.4,0,0.4,0.8,1.2,1.6},yticklabels={−0.8,−0.4,0.0,0.4,0.8,1.2,1.6}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_20/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=-1.30196443855201,
point meta max=1.76162023984194,
colorbar style={ytick={-1.2,-0.8,-0.4,0,0.4,0.8,1.2,1.6},yticklabels={−1.2,−0.8,−0.4,0.0,0.4,0.8,1.2,1.6}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_20_absolute_value/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=0.00399203225432231,
point meta max=1.76162023984194,
colorbar style={ytick={0.2,0.4,0.6,0.8,1,1.2,1.4,1.6},yticklabels={0.2,0.4,0.6,0.8,1.0,1.2,1.4,1.6}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_21/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=-0.658632650174946,
point meta max=2.4181502610445,
colorbar style={ytick={-0.4,0,0.4,0.8,1.2,1.6,2,2.4},yticklabels={−0.4,0.0,0.4,0.8,1.2,1.6,2.0,2.4}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_21_absolute_value/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=0.000715623565806916,
point meta max=2.4181502610445
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_22/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=-1.71692520435452,
point meta max=1.65206481174827,
colorbar style={ytick={-1.6,-1.2,-0.8,-0.4,2.22044604925031e-16,0.4,0.8,1.2,1.6},yticklabels={−1.6,−1.2,−0.8,−0.4,0.0,0.4,0.8,1.2,1.6}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_22_absolute_value/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=0.00113539476025557,
point meta max=1.71692520435452,
colorbar style={ytick={0.2,0.4,0.6,0.8,1,1.2,1.4,1.6},yticklabels={0.2,0.4,0.6,0.8,1.0,1.2,1.4,1.6}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_23/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=-1.66027549230531,
point meta max=1.00315622612834,
colorbar style={ytick={-1.5,-1.2,-0.9,-0.6,-0.3,0,0.3,0.6,0.9},yticklabels={−1.5,−1.2,−0.9,−0.6,−0.3,0.0,0.3,0.6,0.9}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_23_absolute_value/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=0.00261054653674416,
point meta max=1.66027549230531,
colorbar style={ytick={0.2,0.4,0.6,0.8,1,1.2,1.4,1.6},yticklabels={0.2,0.4,0.6,0.8,1.0,1.2,1.4,1.6}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_24/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=-1.50181829645038,
point meta max=1.44929408840835,
colorbar style={ytick={-1.2,-0.8,-0.4,0,0.4,0.8,1.2},yticklabels={−1.2,−0.8,−0.4,0.0,0.4,0.8,1.2}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_24_absolute_value/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=0.00152538258220629,
point meta max=1.50181829645038,
colorbar style={ytick={0.2,0.4,0.6,0.8,1,1.2,1.4},yticklabels={0.2,0.4,0.6,0.8,1.0,1.2,1.4}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_25/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=-0.930197720551956,
point meta max=1.41404896433203,
colorbar style={ytick={-0.75,-0.5,-0.25,-1.11022302462516e-16,0.25,0.5,0.75,1,1.25},yticklabels={−0.75,−0.50,−0.25,0.00,0.25,0.50,0.75,1.00,1.25}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_25_absolute_value/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=0.000608248044037808,
point meta max=1.41404896433203,
colorbar style={ytick={0.15,0.3,0.45,0.6,0.75,0.9,1.05,1.2,1.35},yticklabels={0.15,0.30,0.45,0.60,0.75,0.90,1.05,1.20,1.35}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_26/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=-0.877640924008896,
point meta max=1.784155420959,
colorbar style={ytick={-0.6,-0.3,0,0.3,0.6,0.9,1.2,1.5},yticklabels={−0.6,−0.3,0.0,0.3,0.6,0.9,1.2,1.5}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_26_absolute_value/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=0.000540607234836609,
point meta max=1.784155420959,
colorbar style={ytick={0.2,0.4,0.6,0.8,1,1.2,1.4,1.6},yticklabels={0.2,0.4,0.6,0.8,1.0,1.2,1.4,1.6}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_27/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=-2.55540257014218,
point meta max=1.95710763368697,
colorbar style={ytick={-2.5,-2,-1.5,-1,-0.5,-4.44089209850063e-16,0.5,1,1.5},yticklabels={−2.5,−2.0,−1.5,−1.0,−0.5,0.0,0.5,1.0,1.5}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_27_absolute_value/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=0.00032642333206601,
point meta max=2.55540257014218,
colorbar style={ytick={0.3,0.6,0.9,1.2,1.5,1.8,2.1,2.4},yticklabels={0.3,0.6,0.9,1.2,1.5,1.8,2.1,2.4}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_28/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=-1.15501332862014,
point meta max=1.31188502869904,
colorbar style={ytick={-0.9,-0.6,-0.3,0,0.3,0.6,0.9,1.2},yticklabels={−0.9,−0.6,−0.3,0.0,0.3,0.6,0.9,1.2}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_28_absolute_value/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=0.00233560215553975,
point meta max=1.31188502869904,
colorbar style={ytick={0.15,0.3,0.45,0.6,0.75,0.9,1.05,1.2},yticklabels={0.15,0.30,0.45,0.60,0.75,0.90,1.05,1.20}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_29/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=-2.68355447426438,
point meta max=1.25326385349035
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_29_absolute_value/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=0.00233109391629771,
point meta max=2.68355447426438,
colorbar style={ytick={0.3,0.6,0.9,1.2,1.5,1.8,2.1,2.4},yticklabels={0.3,0.6,0.9,1.2,1.5,1.8,2.1,2.4}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_2_absolute_value/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
%colorbar,
xtick=\empty,
ytick=\empty,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=0.00927264303043416,
point meta max=1.81756495874524,
colorbar style={ytick={0.2,0.4,0.6,0.8,1,1.2,1.4,1.6,1.8},yticklabels={0.2,0.4,0.6,0.8,1.0,1.2,1.4,1.6,1.8}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_2_absolute_value/filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_3/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=-1.65394239438446,
point meta max=0.678761837698054
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_30/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=-3.25901881960453,
point meta max=1.69389545917511,
colorbar style={ytick={-3,-2.4,-1.8,-1.2,-0.6,-4.44089209850063e-16,0.600000000000001,1.2},yticklabels={−3.0,−2.4,−1.8,−1.2,−0.6,0.0,0.6,1.2}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_30_absolute_value/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=0.00172742110529835,
point meta max=3.25901881960453,
colorbar style={ytick={0.4,0.8,1.2,1.6,2,2.4,2.8,3.2},yticklabels={0.4,0.8,1.2,1.6,2.0,2.4,2.8,3.2}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_31/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=-2.78548155538738,
point meta max=1.75383692953736
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_31/normalized_eigenvalues.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=-0.899999999999999,
point meta max=1,
colorbar style={ytick={-0.8,-0.6,-0.4,-0.2,0,0.2,0.4,0.6,0.8,1},yticklabels={−0.8,−0.6,−0.4,−0.2,0.0,0.2,0.4,0.6,0.8,1.0}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {normalized_eigenvalues1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_31_absolute_value/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=0.000832909718155219,
point meta max=2.78548155538738,
colorbar style={ytick={0.3,0.6,0.9,1.2,1.5,1.8,2.1,2.4,2.7},yticklabels={0.3,0.6,0.9,1.2,1.5,1.8,2.1,2.4,2.7}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_3_absolute_value/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
%colorbar,
xtick=\empty,
ytick=\empty,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=0.00171230213050688,
point meta max=1.65394239438446,
colorbar style={ytick={0.2,0.4,0.6,0.8,1,1.2,1.4,1.6},yticklabels={0.2,0.4,0.6,0.8,1.0,1.2,1.4,1.6}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_3_absolute_value/filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_4/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=-0.905080132297426,
point meta max=3.51930867321789,
colorbar style={ytick={-0.5,0,0.5,1,1.5,2,2.5,3,3.5},yticklabels={−0.5,0.0,0.5,1.0,1.5,2.0,2.5,3.0,3.5}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_4_absolute_value/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
%colorbar,
xtick=\empty,
ytick=\empty,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=0.00209638960035366,
point meta max=3.51930867321789,
colorbar style={ytick={0.4,0.8,1.2,1.6,2,2.4,2.8,3.2},yticklabels={0.4,0.8,1.2,1.6,2.0,2.4,2.8,3.2}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_4_absolute_value/filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_5/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=-3.66198687441647,
point meta max=0.595259190449119
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_5_absolute_value/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
%colorbar,
xtick=\empty,
ytick=\empty,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=0.000597093736481562,
point meta max=3.66198687441647,
colorbar style={ytick={0.4,0.8,1.2,1.6,2,2.4,2.8,3.2,3.6},yticklabels={0.4,0.8,1.2,1.6,2.0,2.4,2.8,3.2,3.6}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_5_absolute_value/filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_6/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=-1.84262938687627,
point meta max=0.939377707670725,
colorbar style={ytick={-1.6,-1.2,-0.8,-0.4,2.22044604925031e-16,0.4,0.8},yticklabels={−1.6,−1.2,−0.8,−0.4,0.0,0.4,0.8}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_6_absolute_value/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
%colorbar,
xtick=\empty,
ytick=\empty,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=0.000898283861207845,
point meta max=1.84262938687627,
colorbar style={ytick={0.2,0.4,0.6,0.8,1,1.2,1.4,1.6,1.8},yticklabels={0.2,0.4,0.6,0.8,1.0,1.2,1.4,1.6,1.8}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_6_absolute_value/filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_7/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=-2.21810105764568,
point meta max=1.25033036003411,
colorbar style={ytick={-2,-1.6,-1.2,-0.8,-0.4,0,0.4,0.8,1.2},yticklabels={−2.0,−1.6,−1.2,−0.8,−0.4,0.0,0.4,0.8,1.2}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_7_absolute_value/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
%colorbar,
xtick=\empty,
ytick=\empty,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=2.89986801101242e-05,
point meta max=2.21810105764568,
colorbar style={ytick={0.25,0.5,0.75,1,1.25,1.5,1.75,2},yticklabels={0.25,0.50,0.75,1.00,1.25,1.50,1.75,2.00}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_7_absolute_value/filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_8/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=-0.833072813992201,
point meta max=2.92306307144463
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_8_absolute_value/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
%colorbar,
xtick=\empty,
ytick=\empty,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=0.00295824417232795,
point meta max=2.92306307144463,
colorbar style={ytick={0.3,0.6,0.9,1.2,1.5,1.8,2.1,2.4,2.7},yticklabels={0.3,0.6,0.9,1.2,1.5,1.8,2.1,2.4,2.7}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_8_absolute_value/filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_9/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=-1.84354105636235,
point meta max=2.00882484770808,
colorbar style={ytick={-1.5,-1,-0.5,0,0.5,1,1.5,2},yticklabels={−1.5,−1.0,−0.5,0.0,0.5,1.0,1.5,2.0}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_9_absolute_value/filter.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=-0.5, xmax=19.5,
ymin=-0.5, ymax=19.5,
axis on top,
width=\figurewidth,
height=\figureheight,
%colorbar,
xtick=\empty,
ytick=\empty,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=0.00126891147763753,
point meta max=2.00882484770808
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=19.5, ymax=-0.5] {Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/filter_9_absolute_value/filter1.png};
\end{axis}

\end{tikzpicture}

==> Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/normalized_eigenvalues.tex <==
% This file was created by matplotlib2tikz v0.6.2.
\begin{tikzpicture}

\begin{axis}[
xmin=0, xmax=20,
ymin=0, ymax=20,
axis on top,
width=\figurewidth,
height=\figureheight,
xtick = {0, 8.5, 17},
xticklabels = {-1,0,1},
ytick = {3, 11.5, 20},
yticklabels = {1,0,-1},
xticklabel pos=right,
xlabel near ticks,
axis x line = right,
axis y line = left,
y axis line style = {stealth-},
%colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.5);
  rgb(22pt)=(0,0,1);
  rgb(25pt)=(0,0,1);
  rgb(68pt)=(0,0.86,1);
  rgb(70pt)=(0,0.9,0.967741935483871);
  rgb(75pt)=(0.0806451612903226,1,0.887096774193548);
  rgb(128pt)=(0.935483870967742,1,0.0322580645161291);
  rgb(130pt)=(0.967741935483871,0.962962962962963,0);
  rgb(132pt)=(1,0.925925925925926,0);
  rgb(178pt)=(1,0.0740740740740741,0);
  rgb(182pt)=(0.909090909090909,0,0);
  rgb(200pt)=(0.5,0,0)
},
point meta min=-0.899999999999999,
point meta max=1,
colorbar style={ytick={-0.8,-0.6,-0.4,-0.2,0,0.2,0.4,0.6,0.8,1},yticklabels={−0.8,−0.6,−0.4,−0.2,0.0,0.2,0.4,0.6,0.8,1.0}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=0, xmax=17, ymin=20, ymax=3] {Figures/final_results/tikz/synthetic_netflix/2D_spectral_filters/normalized_eigenvalues1.png};
\end{axis};
\node at (-0.1, -0.1) {\tiny $\lambda_r$};
\node at (1.65, 1.45) {\tiny $\lambda_c$};

\end{tikzpicture}

==> sections/Results_.tex <==
\label{sec:results}

\paragraph*{Experimental settings.} 
We closely followed the experimental setup of \cite{rao2015collaborative}, using five standard datasets: Synthetic dataset from \cite{kalofolias2014matrix}, MovieLens \cite{miller2003movielens}, Flixster \cite{jamali2010matrix}, Douban \cite{art:MaZhouLiuLyuKing11RecomSys}, and YahooMusic \cite{dror2012yahoo}. 
%
Classical Matrix Completion (MC) \cite{candes2012exact}, Inductive Matrix Completion (IMC) \cite{jain2013provable,xu2013speedup}, Geometric Matrix Completion (GMC) \cite{kalofolias2014matrix}, and Graph Regularized Alternating Least Squares (GRALS) \cite{rao2015collaborative} were used as baseline methods.  


In all the experiments, we used the following settings for our RGCNNs: Chebyshev polynomials of order $p=5$, outputting $k=32$-dimensional features, LSTM cells with $32$ features and $T=10$ diffusion steps. All the models were implemented in Google TensorFlow and trained using the Adam stochastic optimization algorithm \cite{KingmaB14} with learning rate $10^{-3}$. In factorized models, rank $r=15$ and $10$ was used for the synthetic and real datasets, respectively. 
%
For all methods, hyperparameters were chosen by cross-validation. 

% and equal to 10 for the real datasets.% in all the experiments where a factorized model was involved. The hyper-parameters have been estimated with suitable grid-search for every considered dataset.


\subsection{Synthetic data}
%In order to show the performance of our approach wrt other state-of-the-art techniques, 
We start our experimental evaluation showing the performance of our approach on a small synthetic dataset, in which the user and item graphs have strong communities structure. Though rather simple, such a dataset allows to study the behavior of different algorithms in controlled settings. 
%
%. Our synthetic set of data appears particularly useful for checking the goodness of our proposal: it is low rank, it presents well defined users/movies graphs and it shows a smooth behaviour over the two domains. 
The performance of different matrix completion methods is reported in Table \ref{tab:results-synthetic-netflix}, along with their theoretical complexity. Two different sets of 15\% of entries represented the training set and test set in our experiments.
Our RGCNN model achieves the best accuracy, followed by the separable RGCNN. 
%
%Our recurrent architecture outperforms all the other competitors, showing a RMSE equal to $5 \cdot 10^{-3}$ and $1 \cdot 10^{-2}$ in its Multi-Graph and separable versions (see 
%
Different diffusion time steps of these two models are visualized in Figure \ref{fig:X-evolutions}. 
%for the evolution in time of matrix $\mathbf{X}$). 
%
Figure \ref{fig:convergence-rate} shows the convergence rates of different methods. Figures \ref{fig:MGCNN-spectral-filter} and \ref{fig:GCNN-spectral-filter} depict the spectral filters learnt by the MGCNN and row- and column-GCNNs. 
%
%Figure \ref{fig:RMSE-mult-algs} finally presents the performance produced by the various algorithms with training sets of different sizes.


We repeated the same experiment considering only the column (users) graph to be given. In this setting, the RGCNN cannot be applied, while the sRGCNN has only one GCNN applied on the factor $\mathbf{H}$, and the other factor $\mathbf{W}$ is free. 
%
Table~\ref{tab:results-synthetic-netflix-one-graph} summarizes the results of this experiment, again, showing that our approach performs the best. 

%To evaluate the robustness of our solution, RGCNN has been also evaluated considering only one of the two graphs. We discarded the movies graph located in our Netflix dataset and we trained our model exploiting just the users domain (matrix $H$ has been directly trained in this case). To avoid overfitting and produce successful results, Eq. (\ref{eq:Dir}) has been modified adding a further regularization term represented by the Frobenius norm of matrix $H$. The results we obtained are reported in Table \ref{tab:results-synthetic-netflix-one-graph}. Again, our approach outperforms the competitor, achieving a RMSE equal to $3.5 \cdot 10^{-2}$ w.r.t. the $4.6 \cdot 10^{-2}$  presented by GRALS. %In Figure \ref{}, we show the convergence rate presented by the various approaches. RGCNN appears as the fastest solution to achieve a valuable minimum. 


\input{figuresfinal_results/tikz/synthetic_netflix/evolutions_X_RGCNN_sRGCNN.tex}

\begin{table}[!ht]
\caption{
Comparison of different matrix completion methods using {\it users+items graphs} in terms of number of parameters (optimization variables) and computational complexity order (operations per iteration). Rightmost column shows the RMS error on Synthetic dataset. 
%Results obtained over the Synthetic Netflix dataset exploiting both the users and movies graphs (\#OPTI = Number of Operations per Training Iteration).
}
\label{tab:results-synthetic-netflix}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lccc}
\hline
\abovespace\belowspace
Method & Parameters & Complexity & RMSE\\
\hline
\abovespace
GMC   & $m n $ & $m n$ & 0.3693   \\
GRALS & $m+n$ & $m+n$ & 0.0114 \\
{\bf RGCNN}    & $\mathbf{1}$ & $\mathbf{m n}$ & {\bf 0.0053} \\
{\bf  sRGCNN}  & $\mathbf{1}$ &$\mathbf{m+n}$ & {\bf 0.0106} \\
%\hline
%GRALS\textsubscript{1 graph}& 0.045169 & O(n+m) & O(n+m) \\
%sRGCNN\textsubscript{1 graph} & 0.036156 & O(1) & O(n+m) \\
\hline
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

\begin{table}[!ht]
\caption{Comparison of different matrix completion methods using {\it users graph only} in terms of number of parameters (optimization variables) and computational complexity order (operations per iteration). Rightmost column shows the RMS error on Synthetic dataset.}
\label{tab:results-synthetic-netflix-one-graph}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lccc}
\hline
\abovespace\belowspace
Method & Parameters & Complexity & RMSE \\
\hline
\abovespace
%MC   & 0.36929   & O(n$\cdot$m) & O(n$\cdot$m)\\
%GRALS & 0.01139 & O(n+m) & O(n+m)\\
%sRGCNN  & 0.01056 & O(1) &O(n+m)\\
%RGCNN    & 0.00611 & O(1) & O(n$\cdot$m)\\
%\hline
GRALS & $m+n$ & $m+n$  & 0.0452 \\
{\bf sRGCNN} & $\mathbf{m}$ & $\mathbf{m+n}$ & {\bf 0.0362}\\
\hline
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}


\begin{figure}[!ht]
\setlength\figureheight{5.5cm}
\setlength\figurewidth{8.5cm}
\input{figuresfinal_results/tikz/synthetic_netflix/convergence_rate/convergence_rate.tex}
\vspace{-5mm}
\caption{Convergence rates of the tested algorithms over the Synthetic Netflix dataset.}
\label{fig:convergence-rate}
\end{figure}

%\begin{figure}[!ht]
%\setlength\figureheight{5.5cm}
%\setlength\figurewidth{8.5cm}
%\input{figuresfinal_results/tikz/synthetic_netflix/RMSE_different_training_sets/RMSE_multiple_training_sets.tex}
%\vspace{-5mm}
%\caption{Performance produced by the various algorithms with training sets of different sizes.}
%\label{fig:RMSE-mult-algs}
%\end{figure}


\begin{figure}[!ht]
\centering
\begin{minipage}[b]{0.2\linewidth}
\hspace*{-0.4cm}\raisebox{-0.1cm}{
\setlength\figureheight{3.2cm}
\setlength\figurewidth{3.2cm}
\input{figuresfinal_results/tikz/synthetic_netflix/2D_spectral_filters/filter_0_absolute_value/filter_big.tex}
%\input{figuresfinal_results/tikz/synthetic_netflix/2D_spectral_filters/normalized_eigenvalues.tex}
}
\end{minipage}
\hfill
\begin{minipage}[b]{0.73\linewidth}
\setlength\figureheight{2.7cm}
\setlength\figurewidth{2.98cm}
\begin{tikzpicture}
\begin{groupplot}[
     group style = {group size = 4 by 2, horizontal sep=0.1cm, vertical sep=0.1cm}]
     
\input{figuresfinal_results/tikz/synthetic_netflix/2D_spectral_filters/filter_0_absolute_value/filter_.tex}
\input{figuresfinal_results/tikz/synthetic_netflix/2D_spectral_filters/filter_1_absolute_value/filter_.tex}
\input{figuresfinal_results/tikz/synthetic_netflix/2D_spectral_filters/filter_2_absolute_value/filter_.tex}
\input{figuresfinal_results/tikz/synthetic_netflix/2D_spectral_filters/filter_3_absolute_value/filter_.tex}

\input{figuresfinal_results/tikz/synthetic_netflix/2D_spectral_filters/filter_4_absolute_value/filter_.tex}
\input{figuresfinal_results/tikz/synthetic_netflix/2D_spectral_filters/filter_5_absolute_value/filter_.tex}
\input{figuresfinal_results/tikz/synthetic_netflix/2D_spectral_filters/filter_6_absolute_value/filter_.tex}
\input{figuresfinal_results/tikz/synthetic_netflix/2D_spectral_filters/filter_7_absolute_value/filter_.tex}
%\input{figuresfinal_results/tikz/synthetic_netflix/2D_spectral_filters/filter_1_absolute_value/filter_.tex}
%\input{figuresfinal_results/tikz/synthetic_netflix/2D_spectral_filters/filter_1_absolute_value/filter_.tex}
  \end{groupplot}
\end{tikzpicture}
\end{minipage}
\caption{Absolute value of the first 8 spectral filters learnt by our bidimensional convolution. On the left the first filter with the reference axes associated to the row and column graph eigenvalues.}
\label{fig:MGCNN-spectral-filter}
\end{figure}


\begin{figure}[!h]
\setlength\figureheight{5.5cm}
\setlength\figurewidth{8.5cm}
\input{figuresfinal_results/tikz/synthetic_netflix/cheb_response_2_different_conv/unique_plot.tex}
%\input{figuresfinal_results/tikz/synthetic_netflix/cheb_response_2_different_conv/row_filters/filter.tex}
%\input{figuresfinal_results/tikz/synthetic_netflix/cheb_response_2_different_conv/col_filters/filter.tex}
\vspace{-2mm}
\caption{Absolute value of the first four spectral filters learned by the user (solid) and items (dashed) GCNNs. }
\label{fig:GCNN-spectral-filter}
\end{figure}



\subsection{Real data}


Following \cite{rao2015collaborative}, we evaluated the proposed approach on the MovieLens, Flixster, Douban and YahooMusic datasets.  
%Different graphs constructions have been exploited for evaluating the various approaches in different operative conditions. 
%
For the MovieLens dataset we constructed the user and item (movie) graphs as unweighted 10-nearest neighbor graphs in the space of user and movie features, respectively. 
%
For Flixster, the user and item graphs were constructed from the scores of the original matrix. On this dataset, we also performed an experiment using only the users graph. 
%
%two 10-NN graphs from the side information available on users and movies. For the Flixster dataset we estimated two 10-NN graphs from the scores available in the original matrix and we evaluated our model assuming to have both of them and just the users domain. 
%
For the Douban dataset, we used only the user graph (the provided social network of the user). 
%
For the YahooMusic dataset, we used only the item graph, constructed with unweighted 10-nearest neighbors in the space of item features (artists, albums, and genres). 
%
For the latter three datasets, we used a sub-matrix of $3000 \times 3000$ entries for evaluating the performance. 

Tables~\ref{tab:results-movielens} and~\ref{tab:other-datasets} summarize the performance of different methods. RGCNN outperforms the competitors in all the experiments. 

%We trained our model for 10k iterations while GRALS for 50k, due to the different convergence rate presented in Figure \ref{fig:convergence-rate}. Hyperparameters have been estimated by cross-validation, training the models respectively for 5k and 25k iterations.% and validating the final $X$ over a portion of the training set.

\begin{table}[!h]
\caption{Performance (RMS error) of different matrix completion methods on the MovieLens dataset.\vspace{-2.25mm}}
\label{tab:results-movielens}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lc}
\hline
\abovespace\belowspace
Method & RMSE \\
\hline
\abovespace 
Global Mean & 1.154\\
User Mean & 1.063\\
Movie Mean & 1.033\\
MC \cite{candes2012exact} & 0.973\\
IMC \cite{jain2013provable,xu2013speedup} & 1.653\\
GMC  \cite{kalofolias2014matrix} & 0.996\\
%\hline
GRALS \cite{rao2015collaborative} & 0.945\\
{\bf sRGCNN} & {\bf 0.929} \\
\hline
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

%\begin{table}[!ht]
%\caption{Results on several datasets.}
%\label{tab:other-datasets}
%\vskip 0.15in
%\begin{center}
%\begin{small}
%\begin{sc}
%\begin{tabular}{lccc}
%\hline
%\abovespace\belowspace
%Method & Flixster & Douban & Yahoo Music \\
%\hline
%\abovespace 
%FMC & 1.1712(1.2447) & 0.8554 & 38.0423\\ 
%sRGCNN & 0.9258 & - & - \\
%sRGCNN\textsubscript{1 graph} & - & 0.8539 & 22.4149 \\
%\hline
%\end{tabular}
%\end{sc}
%\end{small}
%\end{center}
%\vskip -0.1in
%\end{table}


\begin{table}[!h]
\caption{
Matrix completion results on several datasets (RMS error). For Douban and YahooMusic, a single graph (of users and items, respectively) was used. For Flixter, two settings are shown: users+items graphs / only users graph. \vspace{-2.25mm} 
}
\label{tab:other-datasets}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lccc}
\hline
\abovespace\belowspace
Method & Flixster & Douban & YahooMusic \\
\hline
\abovespace 
%FMC & 1.1712(1.2447) & 0.8554 & 38.0423\\ 
GRALS & 1.3126 / 1.2447 & 0.8326 & 38.0423\\ 
{\bf sRGCNN} & {\bf 1.1788} / {\bf 0.9258} & {\bf 0.8012} & {\bf 22.4149} \\
%sRGCNN\textsubscript{1 graph} & - & 0.8539 & 22.4149 \\
\hline
\end{tabular}
\end{sc}
\end{small}
\end{center}
%\vskip -0.1in
\end{table}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%
%\begin{figure*}[!ht]
%\centering
%\setlength\figureheight{2.6cm}
%\setlength\figurewidth{3.05cm}
%
%\begin{minipage}[h]{1.0\linewidth}
%\vspace{1mm}
%\footnotesize
%%\fontsize{7}{5} \selectfont
%\vspace{-3mm}
%\begin{minipage}[h]{0.085\linewidth}
%\center
%t = 0
%\end{minipage}
%\hfill
%\begin{minipage}[h]{0.085\linewidth}
%\center
%1
%\end{minipage}
%\hfill
%\begin{minipage}[h]{0.085\linewidth}
%\center
%2
%\end{minipage}
%\hfill
%\begin{minipage}[h]{0.085\linewidth}
%\center
%3
%\end{minipage}
%\hfill
%\begin{minipage}[h]{0.085\linewidth}
%\center
%4
%\end{minipage}
%\hfill
%\begin{minipage}[h]{0.085\linewidth}
%\center
%5
%\end{minipage}
%\hfill
%\begin{minipage}[h]{0.085\linewidth}
%\center
%6
%\end{minipage}
%\hfill
%\begin{minipage}[h]{0.085\linewidth}
%\center
%7
%\end{minipage}
%\hfill
%\begin{minipage}[h]{0.085\linewidth}
%\center
%8
%\end{minipage}
%\hfill
%\begin{minipage}[h]{0.085\linewidth}
%\center
%9
%\end{minipage}
%\hfill
%\begin{minipage}[h]{0.085\linewidth}
%\center
%10
%\end{minipage}
%\end{minipage}
%\begin{tikzpicture}
%\begin{groupplot}[
%     group style = {group size = 11 by 1, horizontal sep=0.1cm}]
%\input{figuresfinal_results/tikz/synthetic_netflix/evolutions_X/time_0/X.tex}
%\input{figuresfinal_results/tikz/synthetic_netflix/evolutions_X/time_1/X.tex}
%\input{figuresfinal_results/tikz/synthetic_netflix/evolutions_X/time_2/X.tex}
%\input{figuresfinal_results/tikz/synthetic_netflix/evolutions_X/time_3/X.tex}
%\input{figuresfinal_results/tikz/synthetic_netflix/evolutions_X/time_4/X.tex}
%\input{figuresfinal_results/tikz/synthetic_netflix/evolutions_X/time_5/X.tex}
%\input{figuresfinal_results/tikz/synthetic_netflix/evolutions_X/time_6/X.tex}
%\input{figuresfinal_results/tikz/synthetic_netflix/evolutions_X/time_7/X.tex}
%\input{figuresfinal_results/tikz/synthetic_netflix/evolutions_X/time_8/X.tex}
%\input{figuresfinal_results/tikz/synthetic_netflix/evolutions_X/time_9/X.tex}
%\input{figuresfinal_results/tikz/synthetic_netflix/evolutions_X/time_10/X.tex}
%  \end{groupplot}
%\end{tikzpicture}
%\begin{minipage}[h]{1.0\linewidth}
%%\fontsize{7}{5} \selectfont
%\footnotesize
%\vspace{-3mm}
%\begin{minipage}[h]{0.085\linewidth}
%\center
%%RMSE = 
%2.26
%\end{minipage}
%\hfill
%\begin{minipage}[h]{0.085\linewidth}
%\center
% 1.89
%\end{minipage}
%\hfill
%\begin{minipage}[h]{0.085\linewidth}
%\center
% 1.60
%\end{minipage}
%\hfill
%\begin{minipage}[h]{0.085\linewidth}
%\center
% 1.78
%\end{minipage}
%\hfill
%\begin{minipage}[h]{0.085\linewidth}
%\center
% 1.31
%\end{minipage}
%\hfill
%\begin{minipage}[h]{0.085\linewidth}
%\center
% 0.52
%\end{minipage}
%\hfill
%\begin{minipage}[h]{0.085\linewidth}
%\center
% 0.48
%\end{minipage}
%\hfill
%\begin{minipage}[h]{0.085\linewidth}
%\center
% 0.63
%\end{minipage}
%\hfill
%\begin{minipage}[h]{0.085\linewidth}
%\center
% 0.38
%\end{minipage}
%\hfill
%\begin{minipage}[h]{0.085\linewidth}
%\center
% 0.07
%\end{minipage}
%\hfill
%\begin{minipage}[h]{0.085\linewidth}
%\center
% 0.01
%\end{minipage}
%\end{minipage}
%\begin{tikzpicture}
%\begin{groupplot}[
%     group style = {group size = 11 by 1, horizontal sep=0.1cm}]
%\input{figuresfinal_results/tikz/synthetic_netflix/evolutions_X_2_diff_conv/time_0/X.tex}
%\input{figuresfinal_results/tikz/synthetic_netflix/evolutions_X_2_diff_conv/time_1/X.tex}
%\input{figuresfinal_results/tikz/synthetic_netflix/evolutions_X_2_diff_conv/time_2/X.tex}
%\input{figuresfinal_results/tikz/synthetic_netflix/evolutions_X_2_diff_conv/time_3/X.tex}
%\input{figuresfinal_results/tikz/synthetic_netflix/evolutions_X_2_diff_conv/time_4/X.tex}
%\input{figuresfinal_results/tikz/synthetic_netflix/evolutions_X_2_diff_conv/time_5/X.tex}
%\input{figuresfinal_results/tikz/synthetic_netflix/evolutions_X_2_diff_conv/time_6/X.tex}
%\input{figuresfinal_results/tikz/synthetic_netflix/evolutions_X_2_diff_conv/time_7/X.tex}
%\input{figuresfinal_results/tikz/synthetic_netflix/evolutions_X_2_diff_conv/time_8/X.tex}
%\input{figuresfinal_results/tikz/synthetic_netflix/evolutions_X_2_diff_conv/time_9/X.tex}
%\input{figuresfinal_results/tikz/synthetic_netflix/evolutions_X_2_diff_conv/time_10/X.tex}
%  \end{groupplot}
%\end{tikzpicture}
%\begin{minipage}[h]{1.0\linewidth}
%%\fontsize{7}{5} \selectfont
%\footnotesize
%\vspace{-3mm}
%\begin{minipage}[h]{0.085\linewidth}
%\center
% %RMSE = 
% 1.15
%\end{minipage}
%\hfill
%\begin{minipage}[h]{0.085\linewidth}
%\center
% 1.04
%\end{minipage}
%\hfill
%\begin{minipage}[h]{0.085\linewidth}
%\center
% 0.94
%\end{minipage}
%\hfill
%\begin{minipage}[h]{0.085\linewidth}
%\center
% 0.89
%\end{minipage}
%\hfill
%\begin{minipage}[h]{0.085\linewidth}
%\center
% 0.84
%\end{minipage}
%\hfill
%\begin{minipage}[h]{0.085\linewidth}
%\center
% 0.76
%\end{minipage}
%\hfill
%\begin{minipage}[h]{0.085\linewidth}
%\center
% 0.69
%\end{minipage}
%\hfill
%\begin{minipage}[h]{0.085\linewidth}
%\center
% 0.49
%\end{minipage}
%\hfill
%\begin{minipage}[h]{0.085\linewidth}
%\center
% 0.27
%\end{minipage}
%\hfill
%\begin{minipage}[h]{0.085\linewidth}
%\center
% 0.11
%\end{minipage}
%\hfill
%\begin{minipage}[h]{0.085\linewidth}
%\center
% 0.01
%\end{minipage}
%\end{minipage}
%
%\caption{Evolution of the matrix $\mathbf{X}^{(t)}$ with our architecture using full matrix completion model RGCNN (top) and factorized matrix completion model sRGCNN (bottom). Numbers indicate the RMS error. 
%}
%\label{fig:X-evolutions}
%\end{figure*}




%
%\begin{figure}[!ht]
%\centering
%\begin{minipage}[b]{1.0\linewidth}
%	
%	\setlength\figureheight{5cm}
%	\setlength\figurewidth{9cm}
%	\input{figuresfinal_results/tikz/synthetic_netflix/supervised_model/supervised_model.tex}
%   % \includegraphics[width=\linewidth]{figuresfinal_results/supervised_model_factorized_netflix.pdf}
%\end{minipage}
%\hfill
%\begin{minipage}[b]{1.0\linewidth}
%	\setlength\figureheight{5cm}
%	\setlength\figurewidth{9cm}
%	\input{figuresfinal_results/tikz/movielens/supervised_model_factorized.tex}
%    %\includegraphics[width=\linewidth]{figuresfinal_results/supervised_model_factorized_movielens.pdf}
%\end{minipage}
%
%   
%\caption{Reconstructed matrices for the Synthetic Netflix with our multi-graph convolution and for the MovieLens datasets with our factorized approach.}
%\label{fig:X-norm-evolutions}
%\end{figure}


